DGI: Easy and Efficient Inference for GNNs

While many systems have been developed to train Graph Neural Networks (GNNs), efficient model inference and evaluation remain to be addressed. For instance, using the widely adopted node-wise approach, model evaluation can account for up to 94% of the time in the end-to-end training process due to neighbor explosion, which means that a node accesses its multi-hop neighbors. On the other hand, layer-wise inference avoids the neighbor explosion problem by conducting inference layer by layer such that the nodes only need their one-hop neighbors in each layer. However, implementing layer-wise inference requires substantial engineering efforts because users need to manually decompose a GNN model into layers for computation and split workload into batches to fit into device memory. In this paper, we develop Deep Graph Inference (DGI) -- a system for easy and efficient GNN model inference, which automatically translates the training code of a GNN model for layer-wise execution. DGI is general for various GNN models and different kinds of inference requests, and supports out-of-core execution on large graphs that cannot fit in CPU memory. Experimental results show that DGI consistently outperforms layer-wise inference across different datasets and hardware settings, and the speedup can be over 1,000x.

==> deperated/deperated_6_evaluation.tex <==
\section{Evaluation}
\label{sec:eval}

\begin{table*}[h]
  \footnotesize
  \caption{Graphs used in the experiments.}
  \label{tab:evaluation-datasets}
  \centering
%   \fontsize{8}{11}\selectfont 
  \begin{tabular}{cccccc}
    \toprule
    \textbf{Name} & \textbf{Nodes} & \textbf{Edges} & \textbf{Input Dim.} & \textbf{Average Degree} & \textbf{Total Size} \\
    \midrule
    OGBN-Products & 2,449,029  & 126,167,309 & 100 & 51.5 & 2.11 GB    \\
    Friendster & 65,608,366	& 3,612,134,270 & 128 & 55.0	& 58.20 GB     \\
    OGBN-Papers100M & 111,059,956 & 1,726,745,828 & 100 & 15.5 & 64.96 GB \\
    \bottomrule
  \end{tabular}
\end{table*}


%\begin{table}
%	\centering
% 	\fontsize{8}{11}\selectfont    %{字体尺寸}{行距}
%	\caption{Execution time of node-wise inference and \sys (in seconds) for the %\textit{OGBN-Products} graph.}
%	\label{tab:layer-wise comparison}
%	\begin{tabular}{c|ccc|ccc|ccc}
%		%\toprule
%		%  \cr
%		\cmidrule(lr){1-10}
%		\textbf{V100-16GB}&
%		\multicolumn{3}{c}{\textbf{GCN}}&\multicolumn{3}{c}{\textbf{GAT}}&\multicolumn{3}{c}{\textbf{JKNet}} \cr
%		\cmidrule(lr){1-10}
%		Number of Layers & 1 & 2 & 3 & 1 & 2 & 3 & 1 & 2 & 3 \cr
%		\cmidrule(lr){1-10}
%		Node-wise & 3.16 & 153 & 7250 & 3.03 & 189 & 9190 & 152 & 7600 &    $\star$ \cr
%		\sys & 2.60 & 4.37 & 6.08 & 2.62 & 5.68 & 8.96 & 4.31 & 6.70 & 9.10  \cr
%		\bottomrule
%	\end{tabular}\vspace{0cm}
	
%	\begin{tabular}{c|ccc|ccc|ccc}
%		%\toprule
%		%  \cr
%		\cmidrule(lr){1-10}
%		\textbf{V100-32GB}&
%		\multicolumn{3}{c}{\textbf{GCN}}&\multicolumn{3}{c}{\textbf{GAT}}&\multicolumn{3}{c}{\textbf{JKNet}} \cr
%		\cmidrule(lr){1-10}
%		Number of Layers & 1 & 2 & 3 & 1 & 2 & 3 & 1 & 2 & 3 \cr
%		\cmidrule(lr){1-10}
%		Node-wise & 2.56 & 26.8 & 1689 & 2.63 & 29.4 & 1972 & 70.2 & 1763 &    $\star$ \cr
%		\sys & 1.75 & 3.32 & 4.89 & 1.95 & 4.76 & 7.60 & 3.29 & 5.48 & 7.67  \cr
%		\bottomrule
%	\end{tabular}\vspace{0cm}
%\end{table}

\begin{table*}[h]
	\centering
% 	\fontsize{8}{11}\selectfont    %{字体尺寸}{行距}
    \footnotesize
	\caption{Execution time of node-wise inference and \sys (in seconds) for the \textit{OGBN-Products} graph. ``$\star$" means that inference cannot finish in 10,000 seconds.}
	\label{tab:layer-wise comparison}
	\begin{tabular}{c|ccc|ccc|ccc}
		%\toprule
		%  \cr
		\cmidrule(lr){1-10}
		&
		\multicolumn{3}{c}{\textbf{GCN}}&\multicolumn{3}{c}{\textbf{GAT}}&\multicolumn{3}{c}{\textbf{JKNet}} \cr
		\cmidrule(lr){1-10}
		\# of Layers & 1 & 2 & 3 & 1 & 2 & 3 & 1 & 2 & 3 \cr
		\cmidrule(lr){1-10}
		Node-wise (16GB V100) & 3.16 & 153 & 7250 & 3.03 & 189 & 9190 & 152 & 7600 &    $\star$ \cr
		\sys(16GB V100) & 2.60 & 4.37 & 6.08 & 2.62 & 5.68 & 8.96 & 4.31 & 6.70 & 9.10  \cr
		Node-wise (32GB V100) & 2.56 & 26.8 & 1690 & 2.63 & 29.4 & 1970 & 70.2 & 1760 &    $\star$ \cr
		\sys(32GB V100) & 1.75 & 3.32 & 4.89 & 1.95 & 4.76 & 7.60 & 3.29 & 5.48 & 7.67  \cr
		\bottomrule
	\end{tabular}\vspace{0cm}
\end{table*}

\subsection{Experiment settings} We use 3 state-of-the-art GNN models, GCN~\citep{GCN}, GAT~\citep{GAT}, and JKNet~\citep{JKNet} for evaluation. GCN uses mean pooling to aggregate neighbor embeddings. GAT uses multi-head attention mechanism in neighbor aggregation and we set the number of heads to 2. The final layer of JKNet aggregates neighbor embeddings from all preceding layers. By default, we configure the hidden dimension as 128 and use 3 layers for all the models. We conduct the experiments on three widely used public graph datasets: OGBN-Products and OGBN-Papers100M from Open Graph Benchmark~\citep{ogbn} and Friendster~\citep{snap} social network. Their network statistics are reported in Table~\ref{tab:evaluation-datasets}, where the total size includes both graph structure and node features. Both DGI and the baselines are implemented in Deep Graph Library (DGL)~\citep{dgl}. Experiments are conducted on two different machines. One machine has an Intel(R) Xeon(R) E5-2686 CPU with 96 cores, 488 GB main memory, and one NVIDIA V100 GPU with 16GB HBM (denoted as V100-16GB). The other machine has an Intel(R) Xeon(R) Gold 6126 CPU with 24 cores, 1.5TB main memory, and one NVIDIA V100 with 32GB GPU HBM (V100-32GB). The two machines have sufficient main memory to store all data, and we use them as their GPUs have different HBM capacities. 


\subsection{Comparison with node-wise inference} We first compare the execution time of node-wise inference and \sys on the smallest \textit{OGBN-Products} graph in Table~\ref{tab:layer-wise comparison}. For the other two graphs, node-wise inference runs out of memory. For node-wise inference, we use a grid search to find the best batch size in terms of inference speed. The results show that the execution time of node-wise inference quickly rises with more layers due to its fundamental issue of repetitive computation. In contrast, the execution time of \sys increases almost linearly with the number of layers as layer-wise inference only accesses one-hop neighbors. As a result, for 3-layer models, \sys can speed up node-wise inference by more than 3 orders of magnitude. Note that node-wise inference and layer-wise inference are equivalent for 1-layer GNN models, and thus the execution time of node-wise inference and \sys are comparable in this case. The shorter inference time of \sys is attributed to node reorder and dynamic batch size control, which we will analyze in more detail. Both node-wise and layer-wise inference performs better as GPU memory size increases because of the use of a larger batch size, which leads to less data transfer from CPU to GPU. Due to the obvious inefficiencies of node-wise inference, we exclude it from the subsequent experiments.




\begin{figure}
  \includegraphics[width=0.5\textwidth]{figures/ablation_study-1.pdf}
  \caption{Speedup of dynamic batch size and node ordering in DGI overusing best static batch size found by profiling.
  %We report the inference speedup over ST baseline Comparison between the inference execution time of \sys and the baselines. As the execution time for different graphs varies in scale, we normalize the execution time w.r.t. ST. The numbers under each dataset are the inference execution time of \sys (in seconds).
  }
  \label{fig:ablation_study}
\end{figure}

% \begin{figure}[htbp]
% \centering
% \begin{minipage}[t]{0.30\textwidth}
% \centering
% \includegraphics[width=4cm]{figures/micro-reorder.pdf}
% \caption{World Map}
% \end{minipage}
% \begin{minipage}[t]{0.30\textwidth}
% \centering
% \includegraphics[width=4cm]{figures/micro-layer.pdf}
% \caption{Concrete and Constructions}
% \end{minipage}
% \begin{minipage}[t]{0.30\textwidth}
% \centering
% \includegraphics[width=4cm]{figures/micro-io.pdf}
% \caption{Concrete and Constructions}
% \end{minipage}
% \end{figure}


\begin{figure}
  \includegraphics[width=0.5\textwidth]{figures/micro-all.pdf}
  \caption{Micro experiments for \sys designs. We use the GCN model and the Friendster graph.}
  \label{fig:micro-all}
\end{figure}

% \begin{table}
% 	\centering
% % 	\fontsize{8}{11}\selectfont    %{字体尺寸}{行距}
% 	\caption{1}
% 	\label{tab:evaluation}
% 	\begin{tabular}{c|ccc|ccc|ccc}
% 		%\toprule
% 		%  \cr
% 		\cmidrule(lr){1-10}
% 		\multirow{2}{*}{}&
% 		\multicolumn{3}{c}{\textbf{GCN}}&\multicolumn{3}{c}{\textbf{GAT}}&\multicolumn{3}{c}{\textbf{JKNet}} \cr
% 		\cmidrule(lr){2-10}
% % 		& Products & Friendster & Papers100M & Products & Friendster & Papers100M & Products & Friendster & Papers100M \cr
% 		\cmidrule(lr){1-10}
% % 		g4dn.8xlarge & 7.11(0.0331) & 3070(2.50) & 1830(1.49) & 10.9(0.0429) & 4510(3.68) & 2840(2.32) & 11.5(0.0470) & 4780(3.90) & 3200(2.61) \cr
%         g4dn.12xlarge & 7.43 & 2660 & 1590 & 12.3 & 3920 & 2350 & 13.4 & 4250 & 2550\cr
%         p3.16xlarge & 6.10 & 584 & 318 & 8.85 & 986 & 606 & 9.27 & 1176 & 664\cr
%         32GB V100 & 5.65 & 719 & 506 & 3.69 & 328 & 236 & 5.79 & 658 & 433\cr
% 		\bottomrule
% 	\end{tabular}\vspace{0cm}
% \end{table}

% \begin{table}
% 	\centering
% % 	\fontsize{8}{11}\selectfont    %{字体尺寸}{行距}
% 	\caption{Execution time and price for different hardware settings. }
% 	\label{tab:evaluation}
% 	\begin{tabular}{c|ccc|ccc|ccc}
% 		%\toprule
% 		%  \cr
% 		\cmidrule(lr){1-10}
% 		\multirow{2}{*}{Plantform}&
% 		\multicolumn{3}{c}{\textbf{Products}}&\multicolumn{3}{c}{\textbf{Friendster}}&\multicolumn{3}{c}{\textbf{Papers100M}} \cr
% 		\cmidrule(lr){2-10}
% 		& GCN & GAT & JKNet & GCN & GAT & JKNet & GCN & GAT & JKNet \cr
% 		\cmidrule(lr){1-10}
% 		g4dn.8xlarge & 7.11 & 10.9 & 11.5 & 3070 & 4510 & 4780 & 1830 & 2840 & 3200 \cr
% 		g4dn.12xlarge & 7.43 & 12.3 & 13.4 & 2660 & 3920 & 4250 & 1590 & 2360 & 2550 \cr
% 		p3.16xlarge & 6.10 & 8.85 & 9.27 & 584 & 986 & 1180 & 318 & 606 & 664   \cr
% 		32GB V100 & 3.69 & 5.65 & 5.79 & 328 & 718 & 658 & 236 & 506 & 433  \cr
% 	\end{tabular}\vspace{0cm}
% 	\begin{tabular}{c|ccc|ccc|ccc}
% 		%\toprule
% 		%  \cr
% 		\cmidrule(lr){1-10}
% 		\multirow{2}{*}{Prices}&
% 		\multicolumn{3}{c}{\textbf{Products  $(*10^{-3})$}}&\multicolumn{3}{c}{\textbf{Friendster}}&\multicolumn{3}{c}{\textbf{Papers100M}} \cr
% 		\cmidrule(lr){2-10}
% 		& GCN & GAT & JKNet & GCN & GAT & JKNet & GCN & GAT & JKNet \cr
% 		\cmidrule(lr){1-10}
% 		g4dn.8xlarge & 5.80 & 8.91 & 9.40 & 2.50 & 3.68 & 3.90 & 1.49 & 2.32 & 2.61 \cr
% 		g4dn.12xlarge & \textbf{2.73} & \textbf{4.53} & \textbf{4.92} & 0.974 & 1.44 & 1.56 & 0.582 & 0.864 & 0.935   \cr
% 		p3.16xlarge & 7.11 & 10.3 & 10.8 & 0.714 & 1.15 & 1.37 & 0.371 & \textbf{0.706} & 0.774   \cr
% 		32GB V100 & 5.48 & 8.39 & 8.60 & \textbf{0.488} & \textbf{1.07} & \textbf{0.977} & \textbf{0.351} & 0.751 & \textbf{0.644}  \cr
% 		\bottomrule
% 	\end{tabular}\vspace{0cm}
% \end{table}


\begin{table*}[h]
	%\fontsize{8}{11}\selectfont    %{字体尺寸}{行距}
	\footnotesize
	\caption{Execution time of \sys (in seconds) on machines with different configurations. Cases that store data on SSD are marked in bold.}
	\label{tab:cost and time}
	\centering
	\scalebox{0.9}{
		\begin{tabular}{c|ccc|ccc|ccc}
			%\toprule
			%  \cr
			\cmidrule(lr){1-10}
			\multirow{2}{*}{Hardware settings }&
			\multicolumn{3}{c}{\textbf{OGBN-Products}}&\multicolumn{3}{c}{\textbf{Friendster}}&\multicolumn{3}{c}{\textbf{OGBN-Papers100M}} \cr
			\cmidrule(lr){2-10}
			& GCN & GAT & JKNet & GCN & GAT & JKNet & GCN & GAT & JKNet \cr
			\cmidrule(lr){1-10}
			\textbf{(M1)} 128 GB RAM + 16 GB T4 & 7.11 & 10.9 & 11.5 & \textbf{3070} & \textbf{4510} & \textbf{4780} & \textbf{1828} & \textbf{2840} & \textbf{3200} \cr
		    \textbf{(M2)} 192 GB RAM + 16 GB T4 & 6.85 & 10.9 & 11.2 & \textbf{2660} & \textbf{3930} & \textbf{4260} & \textbf{1590} & \textbf{2360} & \textbf{2550} \cr
			\textbf{(M3)} 488 GB RAM + 16 GB V100 & 6.10 & 8.85 & 9.27 & 613 & 986 & 1180 & 318 & 606 & 664      \cr
			\textbf{(M4)} 1.5 TB RAM + 32 GB V100& 3.69 & 5.65 & 5.79 & 328 & 719 & 658 & 236 & 506 & 433    \cr
			\bottomrule
		\end{tabular}
	}
	\vspace{0cm}
\end{table*}


\subsection{Effectiveness of node reordering and dynamic batch size control} To evaluate the effectiveness of \sys's system optimizations, we compare with 4 baselines: \textit{0.25ST}, \textit{0.5ST}, \textit{ST}, and \textit{Dynamic}. \textit{ST} uses the best batch size in terms of inference speed found by grid search.
%adopts a static batch size found by searching for the maximum batch  grid search with an interval of 5,000 to find the maximum batch size that avoids OOM.
Note that \textit{ST} is an ideal case as it requires thorough profiling. We also include \textit{0.5ST} and \textit{0.25ST}, which use 0.5 and 0.25 of the \textit{ST} batch size, respectively. %, and are more close to practical scenarios where users choose a small but safe batch size before execution.
The \textit{Dynamic} baseline enables dynamic batch size control but without node reordering optimization. We then compare them with DGI with all the optimizations enabled.

Figure~\ref{fig:ablation_study} shows the speedup over the \textit{ST} baseline on V100-16GB while the results on V100-32GB are similar and included in the supplementary material. \textit{Dynamic} consistently outperforms \textit{ST} baseline, which indicates the effectiveness of dynamic batch size control. To further understand it, we plot the GPU memory consumption of \sys and \sys with only node reordering enabled throughout the inference process (denoted as \textit{ST+Reorder}, in Figure~\ref{fig:micro-all}(a)).
%We can make several observations from Figure~\ref{fig:ablation_study}. First, dynamic batch size control (DBSC) is effective as Dynamic often outperforms ST, which uses an ideal static batch size. To further explore the effect of DBSC, in Figure~\ref{fig:micro-all}(a), we compare the memory utilization of \sys and \textit{Reorder} (which disables DBSC and uses a static batch size).
The results show that \sys can fully utilize GPU memory most of the time except for the initial bootstrap period. In contrast, the static batch size is limited by the memory consumption of large degree nodes (last few batches) and therefore leads to severe under-utilization. Note that batch size has a larger influence on the \textit{OGBN-Products} graph than the \textit{OGBN-Papers100M} graph. This is because \textit{OGBN-Products} is denser (i.e., with larger average node degrees), so a large batch size leads to better input sharing for computing each batch.
%A closer inspection finds that this is because RCMK tends to put nodes with large in-degrees in the last a few batches, and thus these batches require a small batch size to avoid OOM. However, this batch size is too small for the initial batches (which mainly contain nodes with small in-degrees).

Adding node reordering gives another performance boost to DGI. This is because node reordering organizes nodes with similar neighbors into the same batch to reduce the number of neighbor embeddings to be fetched. Figure~\ref{fig:micro-all}(b) further measures the normalized amount of data transferred by different baselines. With node reordering, DGI can save memory traffic by up to 42.2\% and 39.7\% compared to ST and Dynamic, respectively. Finally,  figure~\ref{fig:micro-all}(c) shows that \sys is resilient to more layers and inference time almost scales linearly with the number of layers. 


% \begin{table}
%   \caption{Instances used in the experiments}
%   \label{tab:instances}
%   \centering
%   \fontsize{9}{10}\selectfont 
%   \begin{tabular}{c|cccc}
%     \toprule
%     Name & CPU Memory (GiB) & GPU Type, Count & GPU Memory (GiB) & Price (USD per Hour)\\
%     \midrule
%     g4dn.8xlarge & 128  & 1 Tesla T4 & 16 & 2.938    \\
%     g4dn.12xlarge & 192	& 4 Tesla T4 & 16 & 5.281     \\
%     p3.16xlarge & 488	& 8 Tesla V100 & 16 & 33.552     \\
%     p3dn.24xlarge & 768	& 8 Tesla V100 & 32 & 42.783     \\
%     \bottomrule
%   \end{tabular}
% \end{table}

% \begin{table}
% 	%\fontsize{8}{11}\selectfont    %{字体尺寸}{行距}
% 	\footnotesize
% 	\caption{}
% 	\label{tab:111}
% 	\centering
% 	\scalebox{0.9}{
% 		\begin{tabular}{c|ccc|ccc}
% 			%\toprule
% 			%  \cr
% 			\cmidrule(lr){1-7}
% 			\multirow{2}{*}{Hardware settings }&
% 			\multicolumn{3}{c}{\textbf{OGBN-Products}}&\multicolumn{3}{c}{\textbf{Friendster}} \cr
% 			\cmidrule(lr){2-7}
% 			& GCN & GAT & JKNet & GCN & GAT & JKNet \cr
% 			\cmidrule(lr){1-7}
% 			488 GB RAM + 16 GB V100 & 500k & 250k & 250k & 80k & 20k & 40k       \cr
% 			1.5 TB RAM + 32 GB V100& 1200k & 1000k & 380k & 120k & 50k & 100k    \cr
% 			\bottomrule
% 		\end{tabular}
% 	}
% 	\vspace{0cm}
% \end{table}


%Thus, an interesting question is how to select a proper machine instance to conduct GNN inference. We report such results in Table~\ref{tab:cost and time}, which leads to several observations. First, inference time significantly reduces when switching data storage from SSD to main memory, as shown by Friendster and OGBN-Papers100M. Second, as observed previously, the benefit of using GPU with larger memory is more obvious for denser graphs (e.g., OGBN-Products and Friendster) than sparser graphs (e.g., OGBN-Papers100M). Third, even for the same graph, the benefit of using larger GPU varies for different models. Take OGBN-Papers100M for example, the JKNet has larger speedup than GCN and GAT when switching from M3 to M4. This is because JKNet requires more input than GCN and GAT in the last layer, and thus benefits more from the large batch size enabled by 32GB GPU memory.                




